Public sentiments on the fourth industrial revolution: An unsolicited public opinion poll from Twitter

This paper establishes an empirical baseline of public sentiment toward Fourth Industrial Revolution (4IR) technologies across six European countries during the period 2006--2019, prior to the widespread adoption of generative AI systems. Employing transformer-based natural language processing models on a corpus of approximately 90,000 tweets and news articles, I document a European public sphere increasingly divided in its assessment of technological change: neutral sentiment declined markedly over the study period as citizens sorted into camps of enthusiasm and concern, a pattern that manifests distinctively across national contexts and technology domains. Approximately 6\% of users inhabit echo chambers characterized by sentiment-aligned networks, with privacy discourse exhibiting the highest susceptibility to such dynamics. These findings provide a methodologically rigorous reference point for evaluating how the introduction of ChatGPT and subsequent generative AI systems has transformed public discourse on automation, employment, and technological change. The results carry implications for policymakers seeking to align technological governance with societal values in an era of rapid AI advancement.

==> figures.tex <==
%--------------------------------------------------
% FIGURES FOR 4IR PUBLIC SENTIMENT PAPER
% Include in preamble: \usepackage{pgfplots, tikz}
% \pgfplotsset{compat=1.18}
%--------------------------------------------------

%--------------------------------------------------
% FIGURE 1: Technology Keyword Frequency (Bar Chart)
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    width=0.9\textwidth,
    height=7cm,
    ylabel={Number of Mentions},
    ylabel style={font=\small},
    symbolic x coords={AI, VR, Blockchain, Robot, Cloud, IoT, 5G},
    xtick=data,
    xticklabel style={font=\small},
    yticklabel style={font=\small},
    nodes near coords,
    nodes near coords style={font=\scriptsize, above},
    ymin=0,
    ymax=40000,
    bar width=0.6cm,
    fill=blue!60,
    every node near coord/.append style={rotate=0, anchor=south},
]
\addplot[fill=blue!60, draw=blue!80] coordinates {
    (AI, 16000)
    (VR, 4000)
    (Blockchain, 27000)
    (Robot, 35000)
    (Cloud, 1000)
    (IoT, 4000)
    (5G, 3500)
};
\end{axis}
\end{tikzpicture}
\caption{Frequency of 4IR technology mentions in corpus. Robotics and blockchain dominate public discourse, while cloud computing receives minimal attention.}
\label{fig:keywords}
\end{figure}

%--------------------------------------------------
% FIGURE 2: Sentiment Trends - Newspaper Tweets
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.85\textwidth,
    height=6.5cm,
    xlabel={Year},
    ylabel={Share of Tweets},
    xmin=2013.5, xmax=2019.5,
    ymin=0, ymax=1,
    xtick={2014,2015,2016,2017,2018,2019},
    ytick={0,0.2,0.4,0.6,0.8,1.0},
    legend style={at={(0.98,0.98)}, anchor=north east, font=\small},
    xlabel style={font=\small},
    ylabel style={font=\small},
    xticklabel style={font=\small},
    yticklabel style={font=\small},
    grid=major,
    grid style={gray!30},
]
% Neutral - declining trend
\addplot[color=green!60!black, mark=*, mark size=2pt, thick] coordinates {
    (2014, 0.78) (2015, 0.72) (2016, 0.68) (2017, 0.62) 
    (2018, 0.55) (2019, 0.52)
};
% Positive - increasing trend
\addplot[color=blue!70, mark=square*, mark size=2pt, thick] coordinates {
    (2014, 0.12) (2015, 0.18) (2016, 0.20) (2017, 0.24) 
    (2018, 0.28) (2019, 0.32)
};
% Negative - stable low
\addplot[color=red!70, mark=triangle*, mark size=2pt, thick] coordinates {
    (2014, 0.10) (2015, 0.10) (2016, 0.12) (2017, 0.14) 
    (2018, 0.17) (2019, 0.16)
};
\legend{Neutral, Positive, Negative}
\end{axis}
\end{tikzpicture}
\caption{Temporal evolution of sentiment in newspaper tweets on 4IR technologies (2014--2019). Neutral sentiment declines from approximately 78\% to 52\%, while positive and negative expressions increase.}
\label{fig:sentimentnews}
\end{figure}

%--------------------------------------------------
% FIGURE 3: Sentiment Trends - User Tweets
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.85\textwidth,
    height=6.5cm,
    xlabel={Year},
    ylabel={Share of Tweets},
    xmin=2013.5, xmax=2019.5,
    ymin=0, ymax=1,
    xtick={2014,2015,2016,2017,2018,2019},
    ytick={0,0.2,0.4,0.6,0.8,1.0},
    legend style={at={(0.98,0.98)}, anchor=north east, font=\small},
    xlabel style={font=\small},
    ylabel style={font=\small},
    grid=major,
    grid style={gray!30},
]
% Neutral - declining trend with more volatility
\addplot[color=green!60!black, mark=*, mark size=2pt, thick] coordinates {
    (2014, 0.82) (2015, 0.70) (2016, 0.65) (2017, 0.58) 
    (2018, 0.50) (2019, 0.48)
};
% Positive - increasing trend
\addplot[color=blue!70, mark=square*, mark size=2pt, thick] coordinates {
    (2014, 0.10) (2015, 0.18) (2016, 0.22) (2017, 0.26) 
    (2018, 0.32) (2019, 0.35)
};
% Negative - gradual increase
\addplot[color=red!70, mark=triangle*, mark size=2pt, thick] coordinates {
    (2014, 0.08) (2015, 0.12) (2016, 0.13) (2017, 0.16) 
    (2018, 0.18) (2019, 0.17)
};
\legend{Neutral, Positive, Negative}
\end{axis}
\end{tikzpicture}
\caption{Temporal evolution of sentiment in user tweets on 4IR technologies (2014--2019). User responses exhibit similar polarization patterns to media coverage, with slightly more pronounced shifts.}
\label{fig:sentimentuser}
\end{figure}

%--------------------------------------------------
% FIGURE 4: Sentiment by Country (6 small multiples)
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
% UK
\begin{axis}[
    name=uk,
    width=5.2cm, height=4cm,
    title={United Kingdom},
    title style={font=\small},
    xmin=2009, xmax=2019,
    ymin=0, ymax=1,
    xtick={2010,2015},
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
    legend style={font=\tiny, at={(0.5,-0.25)}, anchor=north},
]
\addplot[green!60!black, mark=*, mark size=1pt, thick] coordinates {
    (2010,0.85)(2012,0.75)(2014,0.65)(2016,0.55)(2018,0.45)
};
\addplot[blue!70, mark=square*, mark size=1pt, thick] coordinates {
    (2010,0.08)(2012,0.15)(2014,0.22)(2016,0.30)(2018,0.38)
};
\addplot[red!70, mark=triangle*, mark size=1pt, thick] coordinates {
    (2010,0.07)(2012,0.10)(2014,0.13)(2016,0.15)(2018,0.17)
};
\end{axis}

% France
\begin{axis}[
    name=france,
    at={(uk.south east)}, anchor=south west, xshift=0.5cm,
    width=5.2cm, height=4cm,
    title={France},
    title style={font=\small},
    xmin=2009, xmax=2019,
    ymin=0, ymax=1,
    xtick={2010,2015},
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
]
\addplot[green!60!black, mark=*, mark size=1pt, thick] coordinates {
    (2010,0.88)(2012,0.78)(2014,0.68)(2016,0.58)(2018,0.50)
};
\addplot[blue!70, mark=square*, mark size=1pt, thick] coordinates {
    (2010,0.07)(2012,0.14)(2014,0.20)(2016,0.28)(2018,0.35)
};
\addplot[red!70, mark=triangle*, mark size=1pt, thick] coordinates {
    (2010,0.05)(2012,0.08)(2014,0.12)(2016,0.14)(2018,0.15)
};
\end{axis}

% Italy
\begin{axis}[
    name=italy,
    at={(france.south east)}, anchor=south west, xshift=0.5cm,
    width=5.2cm, height=4cm,
    title={Italy},
    title style={font=\small},
    xmin=2011, xmax=2019,
    ymin=0, ymax=1,
    xtick={2012,2016},
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
]
\addplot[green!60!black, mark=*, mark size=1pt, thick] coordinates {
    (2012,0.90)(2014,0.80)(2016,0.65)(2018,0.50)
};
\addplot[blue!70, mark=square*, mark size=1pt, thick] coordinates {
    (2012,0.05)(2014,0.12)(2016,0.25)(2018,0.38)
};
\addplot[red!70, mark=triangle*, mark size=1pt, thick] coordinates {
    (2012,0.05)(2014,0.08)(2016,0.10)(2018,0.12)
};
\end{axis}

% Spain
\begin{axis}[
    name=spain,
    at={(uk.south west)}, anchor=north west, yshift=-1.5cm,
    width=5.2cm, height=4cm,
    title={Spain},
    title style={font=\small},
    xmin=2011, xmax=2019,
    ymin=0, ymax=1,
    xtick={2012,2016},
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
]
\addplot[green!60!black, mark=*, mark size=1pt, thick] coordinates {
    (2012,0.85)(2014,0.72)(2016,0.60)(2018,0.48)
};
\addplot[blue!70, mark=square*, mark size=1pt, thick] coordinates {
    (2012,0.10)(2014,0.20)(2016,0.30)(2018,0.40)
};
\addplot[red!70, mark=triangle*, mark size=1pt, thick] coordinates {
    (2012,0.05)(2014,0.08)(2016,0.10)(2018,0.12)
};
\end{axis}

% Germany
\begin{axis}[
    name=germany,
    at={(spain.south east)}, anchor=south west, xshift=0.5cm,
    width=5.2cm, height=4cm,
    title={Germany},
    title style={font=\small},
    xmin=2011, xmax=2019,
    ymin=0, ymax=1,
    xtick={2012,2016},
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
]
\addplot[green!60!black, mark=*, mark size=1pt, thick] coordinates {
    (2012,0.88)(2014,0.78)(2016,0.68)(2018,0.55)
};
\addplot[blue!70, mark=square*, mark size=1pt, thick] coordinates {
    (2012,0.05)(2014,0.10)(2016,0.15)(2018,0.22)
};
\addplot[red!70, mark=triangle*, mark size=1pt, thick] coordinates {
    (2012,0.07)(2014,0.12)(2016,0.17)(2018,0.23)
};
\end{axis}

% Netherlands
\begin{axis}[
    name=netherlands,
    at={(germany.south east)}, anchor=south west, xshift=0.5cm,
    width=5.2cm, height=4cm,
    title={Netherlands},
    title style={font=\small},
    xmin=2011, xmax=2019,
    ymin=0, ymax=1,
    xtick={2012,2016},
    xticklabel style={font=\tiny},
    yticklabel style={font=\tiny},
]
\addplot[green!60!black, mark=*, mark size=1pt, thick] coordinates {
    (2012,0.92)(2014,0.82)(2016,0.72)(2018,0.58)
};
\addplot[blue!70, mark=square*, mark size=1pt, thick] coordinates {
    (2012,0.05)(2014,0.12)(2016,0.20)(2018,0.32)
};
\addplot[red!70, mark=triangle*, mark size=1pt, thick] coordinates {
    (2012,0.03)(2014,0.06)(2016,0.08)(2018,0.10)
};
\end{axis}

\end{tikzpicture}
\caption{Sentiment dynamics by country. All countries exhibit declining neutrality, but trajectories differ: UK shows steepest polarization; Germany exhibits rising negative sentiment; Netherlands maintains higher neutrality.}
\label{fig:countrysent}
\end{figure}

%--------------------------------------------------
% FIGURE 5: Echo Chamber Trends
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.85\textwidth,
    height=6.5cm,
    xlabel={Year},
    ylabel={Share in Echo Chamber},
    xmin=2009, xmax=2019,
    ymin=0, ymax=0.8,
    xtick={2010,2012,2014,2016,2018},
    ytick={0,0.2,0.4,0.6,0.8},
    legend style={at={(0.02,0.98)}, anchor=north west, font=\scriptsize},
    xlabel style={font=\small},
    ylabel style={font=\small},
    grid=major,
    grid style={gray!30},
]
% AI
\addplot[color=blue!70, mark=*, mark size=1.5pt, thick] coordinates {
    (2010,0.05)(2012,0.15)(2014,0.65)(2016,0.20)(2018,0.25)
};
% Blockchain
\addplot[color=orange!80, mark=square*, mark size=1.5pt, thick] coordinates {
    (2012,0.08)(2014,0.55)(2016,0.18)(2018,0.22)
};
% Robot
\addplot[color=green!60!black, mark=triangle*, mark size=1.5pt, thick] coordinates {
    (2010,0.03)(2012,0.12)(2014,0.48)(2016,0.15)(2018,0.20)
};
% IoT
\addplot[color=purple!70, mark=diamond*, mark size=1.5pt, thick] coordinates {
    (2012,0.04)(2014,0.35)(2016,0.12)(2018,0.18)
};
\legend{AI, Blockchain, Robot, IoT}
\end{axis}
\end{tikzpicture}
\caption{Temporal evolution of echo chamber participation by technology. Sharp spike in 2014 across categories coincides with high-profile AI risk warnings and cryptocurrency debates.}
\label{fig:echotrend}
\end{figure}

%--------------------------------------------------
% FIGURE 6: Misinformation Exposure Distribution
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar interval,
    width=0.85\textwidth,
    height=6cm,
    xlabel={Misinformation Exposure Score},
    ylabel={Frequency},
    xmin=0, xmax=1,
    ymin=0, ymax=22000,
    xtick={0,0.2,0.4,0.6,0.8,1.0},
    xticklabel style={font=\small},
    yticklabel style={font=\small},
    xlabel style={font=\small},
    ylabel style={font=\small},
]
\addplot[fill=blue!50, draw=blue!70] coordinates {
    (0.0, 18000) (0.1, 20000) (0.2, 15000) (0.3, 12000) 
    (0.4, 8000) (0.5, 5000) (0.6, 3000) (0.7, 1500) 
    (0.8, 800) (0.9, 400) (1.0, 0)
};
\end{axis}
% Add mean and median lines
\draw[red, thick, dashed] (3.2cm, 0.5cm) -- (3.2cm, 5.5cm) node[above, font=\scriptsize] {Mean=0.26};
\draw[orange, thick, dashed] (4.5cm, 0.5cm) -- (4.5cm, 5.5cm) node[above, font=\scriptsize] {Median=0.37};
\end{tikzpicture}
\caption{Distribution of misinformation exposure scores. The right-skewed distribution indicates most users have low exposure, but a substantial tail exhibits elevated misinformation exposure.}
\label{fig:misinfohist}
\end{figure}

%--------------------------------------------------
% FIGURE 7: Misinformation by Theme (Box Plot)
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.85\textwidth,
    height=6cm,
    boxplot/draw direction=y,
    xlabel={Thematic Domain},
    ylabel={Misinformation Exposure Score},
    xtick={1,2,3,4,5},
    xticklabels={Employment, Environment, Health, Other, Privacy},
    xticklabel style={font=\small},
    yticklabel style={font=\small},
    xlabel style={font=\small},
    ylabel style={font=\small},
    ymin=0, ymax=0.6,
]
% Employment
\addplot+[boxplot prepared={
    lower whisker=0.08,
    lower quartile=0.18,
    median=0.25,
    upper quartile=0.32,
    upper whisker=0.45
}, fill=blue!30] coordinates {};

% Environment
\addplot+[boxplot prepared={
    lower whisker=0.06,
    lower quartile=0.16,
    median=0.24,
    upper quartile=0.30,
    upper whisker=0.42
}, fill=green!30] coordinates {};

% Health
\addplot+[boxplot prepared={
    lower whisker=0.05,
    lower quartile=0.15,
    median=0.24,
    upper quartile=0.31,
    upper whisker=0.44
}, fill=orange!30] coordinates {};

% Other
\addplot+[boxplot prepared={
    lower whisker=0.07,
    lower quartile=0.17,
    median=0.25,
    upper quartile=0.33,
    upper whisker=0.46
}, fill=gray!30] coordinates {};

% Privacy
\addplot+[boxplot prepared={
    lower whisker=0.10,
    lower quartile=0.20,
    median=0.27,
    upper quartile=0.36,
    upper whisker=0.50
}, fill=red!30] coordinates {};

\end{axis}
\end{tikzpicture}
\caption{Misinformation exposure by thematic domain. Privacy discourse exhibits the highest median exposure score, consistent with elevated polarization and echo chamber prevalence in this domain.}
\label{fig:misinfotheme}
\end{figure}

%--------------------------------------------------
% FIGURE 8: Misinformation Temporal Trend
%--------------------------------------------------
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.85\textwidth,
    height=6cm,
    xlabel={Year},
    ylabel={Share with High Misinformation Exposure},
    xmin=2012.5, xmax=2019.5,
    ymin=0, ymax=1,
    xtick={2013,2014,2015,2016,2017,2018,2019},
    ytick={0,0.2,0.4,0.6,0.8,1.0},
    xlabel style={font=\small},
    ylabel style={font=\small},
    xticklabel style={font=\small},
    yticklabel style={font=\small},
    grid=major,
    grid style={gray!30},
]
\addplot[color=red!70, mark=*, mark size=2pt, thick] coordinates {
    (2013, 0.15) (2014, 0.22) (2015, 0.28) (2016, 0.35) 
    (2017, 0.42) (2018, 0.48) (2019, 0.52)
};
% Add trend line
\addplot[color=red!40, thick, dashed, domain=2013:2019] {0.06*x - 120.5};
\end{axis}
\end{tikzpicture}
\caption{Temporal trend in misinformation exposure (2013--2019). The share of users with elevated misinformation exposure more than tripled over the study period, indicating degradation of information environments preceding COVID-19.}
\label{fig:misinfotrend}
\end{figure}
